Local Hypergraph Clustering using Capacity Releasing Diffusion

Local graph clustering is an important machine learning task that aims to find a well-connected cluster near a set of seed nodes. Recent results have revealed that incorporating higher order information significantly enhances the results of graph clustering techniques. The majority of existing research in this area focuses on spectral graph theory-based techniques. However, an alternative perspective on local graph clustering arises from using max-flow and min-cut on the objectives, which offer distinctly different guarantees. For instance, a new method called capacity releasing diffusion (CRD) was recently proposed and shown to preserve local structure around the seeds better than spectral methods. The method was also the first local clustering technique that is not subject to the quadratic Cheeger inequality by assuming a good cluster near the seed nodes. In this paper, we propose a local hypergraph clustering technique called hypergraph CRD (HG-CRD) by extending the CRD process to cluster based on higher order patterns, encoded as hyperedges of a hypergraph. Moreover, we theoretically show that HG-CRD gives results about a quantity called motif conductance, rather than a biased version used in previous experiments. Experimental results on synthetic datasets and real world graphs show that HG-CRD enhances the clustering quality.

==> dgleich-extra.tex <==
\usepackage{ushort}
\newcommand{\cel}[1]{\ushort{#1}}
\newcommand{\cbmat}[1]{\left\{ \begin{matrix} #1 \end{matrix} \right\}}
\newcommand{\csbmat}[1]{\left\{\! \begin{smallmatrix} #1
\end{smallmatrix} \! \right\}}
%\newcommand{\csbmat}[1]{\underline{\sbmat{#1}}}
\newcommand{\smallmath}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\celm}[1]{\cel{\mat{#1}}}
\newcommand{\celv}[1]{\cel{\vec{#1}}}



\newcommand{\calpha}{\ensuremath{\cel{\alpha}}}
\newcommand{\cbeta}{\ensuremath{\cel{\beta}}}
\newcommand{\clambda}{\ensuremath{\cel{\lambda}}}

\newcommand{\cone}{\ensuremath{\cel{1}}}
\newcommand{\ca}{\ensuremath{\cel{a}}}
\newcommand{\cb}{\ensuremath{\cel{b}}}
\newcommand{\cc}{\ensuremath{\cel{c}}}
\newcommand{\cd}{\ensuremath{\cel{d}}}
\newcommand{\ce}{\ensuremath{\cel{e}}}
\newcommand{\cf}{\ensuremath{\cel{f}}}
\newcommand{\cg}{\ensuremath{\cel{g}}}
\newcommand{\ch}{\ensuremath{\cel{h}}}
\newcommand{\ci}{\ensuremath{\cel{i}}}
\newcommand{\cj}{\ensuremath{\cel{j}}}
\newcommand{\ck}{\ensuremath{\cel{k}}}
\newcommand{\cl}{\ensuremath{\cel{l}}}
\newcommand{\cm}{\ensuremath{\cel{m}}}
\newcommand{\cn}{\ensuremath{\cel{n}}}
\newcommand{\co}{\ensuremath{\cel{o}}}
\newcommand{\cp}{\ensuremath{\cel{p}}}
\newcommand{\cq}{\ensuremath{\cel{q}}}
%\newcommand{\cr}{\ensuremath{\cel{r}}}
\newcommand{\cs}{\ensuremath{\cel{s}}}
\newcommand{\ct}{\ensuremath{\cel{t}}}
\newcommand{\cu}{\ensuremath{\cel{u}}}
\newcommand{\cv}{\ensuremath{\cel{v}}}
\newcommand{\cw}{\ensuremath{\cel{w}}}
\newcommand{\cx}{\ensuremath{\cel{x}}}
\newcommand{\cy}{\ensuremath{\cel{y}}}
\newcommand{\cz}{\ensuremath{\cel{z}}}


\newcommand{\cA}{\ensuremath{\cel{A}}}
\newcommand{\cB}{\ensuremath{\cel{B}}}
\newcommand{\cC}{\ensuremath{\cel{C}}}
\newcommand{\cD}{\ensuremath{\cel{D}}}
\newcommand{\cE}{\ensuremath{\cel{E}}}
\newcommand{\cF}{\ensuremath{\cel{F}}}
\newcommand{\cG}{\ensuremath{\cel{G}}}
\newcommand{\cH}{\ensuremath{\cel{H}}}
\newcommand{\cI}{\ensuremath{\cel{I}}}
\newcommand{\cJ}{\ensuremath{\cel{J}}}
\newcommand{\cK}{\ensuremath{\cel{K}}}
\newcommand{\cL}{\ensuremath{\cel{L}}}
\newcommand{\cM}{\ensuremath{\cel{M}}}
\newcommand{\cN}{\ensuremath{\cel{N}}}
\newcommand{\cO}{\ensuremath{\cel{O}}}
\newcommand{\cP}{\ensuremath{\cel{P}}}
\newcommand{\cQ}{\ensuremath{\cel{Q}}}
\newcommand{\cR}{\ensuremath{\cel{R}}}
\newcommand{\cS}{\ensuremath{\cel{S}}}
\newcommand{\cT}{\ensuremath{\cel{T}}}
\newcommand{\cU}{\ensuremath{\cel{U}}}
\newcommand{\cV}{\ensuremath{\cel{V}}}
\newcommand{\cW}{\ensuremath{\cel{W}}}
\newcommand{\cX}{\ensuremath{\cel{X}}}
\newcommand{\cY}{\ensuremath{\cel{Y}}}
\newcommand{\cZ}{\ensuremath{\cel{Z}}}


\newcommand{\cva}{\ensuremath{\celv{a}}}
\newcommand{\cvb}{\ensuremath{\celv{b}}}
\newcommand{\cvc}{\ensuremath{\celv{c}}}
\newcommand{\cvd}{\ensuremath{\celv{d}}}
\newcommand{\cve}{\ensuremath{\celv{e}}}
\newcommand{\cvf}{\ensuremath{\celv{f}}}
\newcommand{\cvg}{\ensuremath{\celv{g}}}
\newcommand{\cvh}{\ensuremath{\celv{h}}}
\newcommand{\cvi}{\ensuremath{\celv{i}}}
\newcommand{\cvj}{\ensuremath{\celv{j}}}
\newcommand{\cvk}{\ensuremath{\celv{k}}}
\newcommand{\cvl}{\ensuremath{\celv{l}}}
\newcommand{\cvm}{\ensuremath{\celv{m}}}
\newcommand{\cvn}{\ensuremath{\celv{n}}}
\newcommand{\cvo}{\ensuremath{\celv{o}}}
\newcommand{\cvp}{\ensuremath{\celv{p}}}
\newcommand{\cvq}{\ensuremath{\celv{q}}}
\newcommand{\cvr}{\ensuremath{\celv{r}}}
\newcommand{\cvs}{\ensuremath{\celv{s}}}
\newcommand{\cvt}{\ensuremath{\celv{t}}}
\newcommand{\cvu}{\ensuremath{\celv{u}}}
\newcommand{\cvv}{\ensuremath{\celv{v}}}
\newcommand{\cvw}{\ensuremath{\celv{w}}}
\newcommand{\cvx}{\ensuremath{\celv{x}}}
\newcommand{\cvy}{\ensuremath{\celv{y}}}
\newcommand{\cvz}{\ensuremath{\celv{z}}}

\providecommand{\cmA}{\ensuremath{\celm{A}}}
\providecommand{\cmB}{\ensuremath{\celm{B}}}
\providecommand{\cmC}{\ensuremath{\celm{C}}}
\providecommand{\cmD}{\ensuremath{\celm{D}}}
\providecommand{\cmE}{\ensuremath{\celm{E}}}
\providecommand{\cmF}{\ensuremath{\celm{F}}}
\providecommand{\cmG}{\ensuremath{\celm{G}}}
\providecommand{\cmH}{\ensuremath{\celm{H}}}
\providecommand{\cmI}{\ensuremath{\celm{I}}}
\providecommand{\cmJ}{\ensuremath{\celm{J}}}
\providecommand{\cmK}{\ensuremath{\celm{K}}}
\providecommand{\cmL}{\ensuremath{\celm{L}}}
\providecommand{\cmM}{\ensuremath{\celm{M}}}
\providecommand{\cmN}{\ensuremath{\celm{N}}}
\providecommand{\cmO}{\ensuremath{\celm{O}}}
\providecommand{\cmP}{\ensuremath{\celm{P}}}
\providecommand{\cmQ}{\ensuremath{\celm{Q}}}
\providecommand{\cmR}{\ensuremath{\celm{R}}}
\providecommand{\cmS}{\ensuremath{\celm{S}}}
\providecommand{\cmT}{\ensuremath{\celm{T}}}
\providecommand{\cmU}{\ensuremath{\celm{U}}}
\providecommand{\cmV}{\ensuremath{\celm{V}}}
\providecommand{\cmW}{\ensuremath{\celm{W}}}
\providecommand{\cmX}{\ensuremath{\celm{X}}}
\providecommand{\cmY}{\ensuremath{\celm{Y}}}
\providecommand{\cmZ}{\ensuremath{\celm{Z}}}

\newcommand{\cmPt}{\cel{\mat{\tilde{P}}}}
\renewcommand{\cmPt}{\mat{\tilde{P}}}

\newcommand{\elm}[1]{\cel{#1}}

==> higher_order_crd.tex <==


\section{A Capacity Releasing Diffusion for Hypergraphs via Motif Matrices} \label{sec:higher_order_crd}

Our main contribution is the HG-CRD algorithm that avoids the motif-weighted adjacency matrix. We begin, however, by describing how CRD can already be combined with the motif-weighted adjacency matrix in the CRD-M algorithm. For three node motifs, this offers a variety of theoretical guarantees, but there are significant biases for larger motifs that we are able to mitigate with our HG-CRD algorithm.

%\subsection{CRD using Motif Adjacency Matrix (CRD-M)}

One straightforward idea to extend capacity releasing diffusion to cluster based on higher order patterns is to construct the motif adjacency matrix $\mW_M$ as described by~\cite{benson2016higher}, where the entry $\mW_M(i, j)$ equals to the number of motif instances that both node $i$ and node $j$ appear in its nodes. After constructing the motif adjacency matrix, we will run the CRD process on the graph represented by the motif adjacency matrix $\mW_M$. As the CRD process does not take into account the weight of the edges, we consider two variations, the first one is to duplicate each edge $(u, v)$ $\mW_M(u, v)$ times. This results in a multigraph, where the CRD algorithm can be easily adapted and the second variation is to multiply the weight of the edge $(u, v)$ used in the CRD process by $\mW_M(u, v)$. We report the second variation in the experimental results as it has the best $F_1$ in all datasets. Based on~\cite{benson2016higher} proof, when the size of the motif is three, then the motif conductance will be equal to the conductance of the graph represented by the motif adjacency matrix. As the CRD process guarantees that the conductance of the returned cluster is $O(\phi)$ where $\phi$ is a parameter input to the algorithm that controls both the maximum flow that can be pushed along each edge and the maximum node level during the push-relabel process. This extension guarantees that when the motif size is three, the motif conductance of the returned cluster is $O(\phi)$. In the rest of the paper, we will propose another extension for higher order capacity releasing diffusion that has a motif conductance guarantee of $O(k \phi)$ for any motif size $k$.

\subsection{A true hypergraph CRD}


%\subsubsection{CRD using Hyperedge-based Flow Idea}

Let $H = (V, \cE)$ be a hypergraph where the hyperedges $\cE$ represent motifs. For this reason, we will use \emph{motif} and \emph{hyperedge} largely interchangeably. The basic idea in CRD is to push flow along edges until a bottleneck emerges. In HG-CRD, the basic idea is the same. We push the flow across hyperedges as much as we can until there is too much excess flow on the nodes, which means nodes are unable to push much flow to hyperedges containing them. This will happen because the algorithm has reached a bottleneck and hence the algorithm has identified the desired cluster with respect to the high order pattern or motif. As such, the HG-CRD procedure is highly algorithmic as it implements a specific procedure to move \emph{flow} around the graph to identify this bottleneck. 

The input to the HG-CRD algorithm is a hypergraph H, a seed node $s$, and parameters $\phi, \tau, t, \alpha$. The parameter $t$ controls the number of iterations of the procedure, which is largely correlated with how large the final set should be. The parameter $\tau$ controls what is too much excess flow on the nodes and the parameter $\alpha$ controls whether we can push flow along the hyperedge or not. The value $\phi$ is the target value of motif conductance to obtain. That is, $\phi$ is an estimate of the bottleneck. Note that much of the theory is in terms of the value of $\phi$, but the algorithm uses the quantity $C = 1/\phi$ in many places instead. The output of the algorithm is the set $A$ representing the cluster of node $s$.

We begin by providing a set of quantities the algorithm manipulates and a simple example.

\subsection{Node and Hyperedge variables in HG-CRD}
Each node $v$ in the graph will have four values associated with it, which are: the degree of the node $\vd_M(V)$, the flow at the node $\vm_M(v)$, the excess flow at the node \textbf{ex}(v), and the node level $\vl(v)$. In the hypergraph, we define the degree as follows: 
\begin{align*}
\vd_M(v) = (k-1) \sum_{e \in \cE} \begin{cases} 1 & v \in e \\ 0 & \text{otherwise.} \end{cases}
\end{align*}
 That is, degree $\vd_M(v)$ of vertex $v$ will be $(k-1) \times~ $ the number of hyperedges containing $v$.

A node $v$ has excess flow if and only if $\vm_M(v) \geq \vd_M(v) + (k-1)$ and in this case we will call node $v$ to be \textit{active}. Additionally, we will define excess of flow $\textbf{ex}(v)$ at node $v$ to be max($\vm_M(v) - \vd_M(v)$, 0) and therefore, we visualize each node $v$ to have a capacity of $\vd_M(v)$ and any extra flow than this is excess. We will also restrict the node level to have a maximum value $h = \frac{3 \text{log} (\ve^T \vm_M)}{\phi}$. If $\vl(v)$ reach $h$, then node $v$ cannot send or receive any flow.

Moreover, each hyperedge $e = (v, u_1, ... u_{k-1})$ will have a capacity $C = \frac{1}{\phi}$, where $\phi$ is a parameter input to the algorithm and $e$ will have a flow value associated with it $\vm_M(e)$, which represents how much flow is pushed along this hyperedge. To determine if we can push more flow through this hyperedge or not, we will have a residual capacity variable with each hyperedge and it will be defined as $r(e) = \text{min}(\vl(v), C) - \vm_M(e)$. In the process, we can push flow through the hyperedge $e = (v, u_1, ... u_{k-1})$ if and only if it is an eligible hyperedge, where an eligible hyperedge is defined as: 
\begin{itemize}
    \item $\vl(v) > \vl(u_i) \text{ for at least } \alpha \text{ } u_i \in e \setminus v$, where $\alpha \in [1, k-1]$.
    \item $r(e) > 0$.
\end{itemize}


%Given a motif $x$, we will construct a hypergraph $H = (V, EH)$, where $V$ is the set of nodes in graph $G$ and $EH$ is the set of hyperedges in graph $G$ enumerated according to the motif $x$.  Formally, let us define the motif-based degree of the node as follows:

\begin{fullwidthtable}
%\fbox{
\noindent\begin{minipage}[h] {0.6\linewidth} 
\label{alg:crd_inner_algorithm}
%\caption{HG-CRD pseudocode.}
\small
\DontPrintSemicolon
\SetAlgoLined
\hspace{0.1cm} \nl \SetKwFunction{Main}{HG-CRD Algorithm}
\Main{G, s, $\phi$, $\tau$, t, $\alpha$} {
	
\hspace{0.1cm} \nl	$\vm_M \leftarrow 0 ;$ $\vm_M(s) \leftarrow \vd_M(s);$ $A \leftarrow \{ \};$ $\phi^* \leftarrow 1$ \;
	
\hspace{0.1cm} \nl	\ForEach{$j = 0, ..., t$} {
	
\hspace{0.1cm} \nl		$\vm_M \leftarrow 2 \vm_M;$ 
		
\hspace{0.1cm} \nl $\vl \leftarrow$ HG-CRD-inner($G$, $\vm_M$, $\phi$,  $\alpha$); 
		
\hspace{0.1cm} \nl		$Kj \leftarrow $ Sweepcut($G$, $\vl$)\;
		
\hspace{0.1cm} \nl		\textbf{if} $\phi_M(Kj) < \phi^*$ \textbf{then} $A \leftarrow Kj;$ $\phi^* \leftarrow \phi_M(Kj)$ \; 

\hspace{0.1cm} \nl $\vm_M \leftarrow \text{min}(\vm_M, \vd_M)$\;
		
\hspace{0.1cm} \nl		\textbf{if} $\ve^T \vm_M \leq \tau (2 \vd_M(s) 2^j)$ \textbf{then} Return $A$ \;
	}

\hspace{0.1cm} \nl    Return $A$ \;
}

 \SetKwFunction{Main}{HG-CRD-inner}

\hspace{0.1cm} \nl \Main{$G$,$\vm_M$, $\phi$, $\alpha$} { 

\hspace{0.1cm} \nl $\vl = 0;$ $\textbf{ex} = 0;$ $Q = \{ v | \vm_M(v) \geq \vd_M(v) + (k-1)\};$ 

\hspace{0.1cm} \nl $h = \frac{3 \text{log} (\ve^T \vm_M)}{\phi}$ \;

	\hspace{0.1cm} \nl \While{Q is not empty}{
		
\hspace{0.1cm} \nl		$v \leftarrow$ Q.get-lowest-level-node(); 
		
\hspace{0.1cm} \nl		$e = (v, u_1, ..., u_{k-1}) \leftarrow $ pick-eligible-hyperedge(v);
		
\hspace{0.1cm} \nl		pushed-flow $\leftarrow false$ \;
        
\hspace{0.1cm} \nl        \If {$e \neq \{ \}$} {

\hspace{0.1cm} \nl  \hspace{-0.1cm} $\Psi = \text{min} (\lfloor \frac{\textbf{ex}(v)}{k-1} \rfloor, r(e), 2 \vd_M(u_i) - \vm_M(u_i) \text{ } \forall u_i);$ 

\hspace{0.1cm} \nl $\vm_M(e) \leftarrow \vm_M(e) + \Psi$ 
    	    
\hspace{0.1cm} \nl    	    $\vm_M(v) \leftarrow \vm_M(v) - (k-1) \Psi; $
    	    
 \hspace{0.1cm} \nl   	    $\vm_M(u) \leftarrow \vm_M(u) + \Psi \text{ } \forall u_i \in e \setminus v$ 		
	    
 \hspace{0.1cm} \nl   		\uIf{$\Psi \neq 0$} { 
  \hspace{0.1cm} \nl  		
    		    pushed-flow $\leftarrow true$; 
    		    
\hspace{0.1cm} \nl    		    \textbf{ex}(v) $\leftarrow$ max($\vm_M(v) - \vd_M(v),0$) \;
    			
 \hspace{0.1cm} \nl   			\textbf{if} $\textbf{ex}(v) < k-1$ \textbf{then } Q.remove(v)  \;
    
 \hspace{0.1cm} \nl   			\For{$u_i \in e$} {
    			
  \hspace{0.1cm} \nl  			\textbf{ex}($u_i$) $\leftarrow$ max($\vm_M(u_i) - \vd_M(u_i),0$) \;
    			
  \hspace{0.1cm} \nl  			\textbf{if} $\textbf{ex}(u_i) \geq (k-1)$ \text { and } $\vl(u_i) < h$ \textbf{then} 
  
  \hspace{0.1cm} \nl Q.add($u_i$)\;
    			}
    			
    		}
		} 
\hspace{0.1cm} \nl		\If{not pushed-flow}  {
			
\hspace{0.1cm} \nl			$\vl(v) \leftarrow \vl(v) + 1$ \textbf{if} $\vl(v)$ == h \textbf{then } Q.remove(v) 
		}
	}
	}
\end{minipage}
%}
%\hfill
\begin{minipage}[h]{0.4\linewidth}
\footnotesize
\centering
\caption{Description of used terms.}
\begin{tabularx}{\linewidth} {p{1.2cm}X}  \toprule
Term & Definition \\
\midrule
$\vd_M(v)$ & motif-based degree of node $v$\\
\addlinespace
$\vm_M(v)$ & flow at node $v$\\
\addlinespace
$\textbf{ex}(v)$ & excess flow at node $v$\\
\addlinespace
$\vl(v)$ & level of node $v$ \\
\addlinespace
$h$ & maximum level of any node\\
\addlinespace
$C$ & maximum capacity of any edge\\
\addlinespace
$\vm_M(e)$ & flow at edge $e$\\
\addlinespace
$r(e)$ & residual capacity of edge $e$\\
\addlinespace
$s$ & seed node\\
\addlinespace
$t$ & maximum number of HG-CRD inner calls\\
\addlinespace
$\tau$ & controls how much is much excess\\
\addlinespace
%Eligible hyperedge (e)  & if its source node has higher level than at least $\alpha$ other nodes in e and $r(e) > 0$ \\
%\addlinespace
$\alpha$ & controls the eligibility of hyperedge \\
\addlinespace
$\phi$ & controls the values of $C$ and $h$ \\ \addlinespace
$\ve$ & vector of all ones\\
\addlinespace
$\text{vol}_M(B)$ & the number of motif instances end points in $B$ \\
\addlinespace
$\text{volM}(B)$ & $\sum_{v \in B} d_M(v)= (k-1) \text{vol}_M(B)$\\
\addlinespace
$\phi_M(B)$ & motif conductance of $B$\\
\addlinespace
$K_j$ & set of nodes in the cluster in the jth iteration\\
\bottomrule
\end{tabularx}
\end{minipage}
\end{fullwidthtable}


\subsection{The high-level algorithm}

The exact algorithm details which are adjusted from the pseudocodes in~\cite{wang2017capacity} to account for the impact of hyperedges, are present in HG-CRD Algorithm. In this section, we summarize the main intuition for the algorithm. At the start, the flow value $\vm_M(s)$ at the seed node $s$ will be equal to $2 \vd_M(s)$ and in each iteration,  HG-CRD will double the flow on each visited node. Each node $v$ that has excess flow picks an \textit{eligible} hyperedge $e$ that contains the node $v$ and sends flow to all other nodes in the hyperedge $e$. After performing an iteration (which we will call it HG-CRD-inner in the pseudocode,) we will remove any excess flow at the nodes (step 8 in pseudocode). If all nodes do not have excess flow in all iterations (no bottleneck is reached yet) and as we double the flow at each iteration $j$, then the total sum of flow at the nodes will be equal to $2 \vd_M(s) 2^j$. However, if the total sum of flow at the nodes is significantly (according to the parameter $\tau$) less than $2 \vd_M(s) 2^j$, then step 8 has removed a lot of flow excess at the nodes because many nodes had flow excess at the end of the iteration. This indicates that the flow was contaminated and we have reached a bottleneck for the cluster. Finally, we will obtain the cluster $A$ by performing a sweep-cut procedure. Sweep-cut is done by sorting the nodes in descending order according to their level values, then evaluating the conductance of each prefix set and returning the cluster with the lowest conductance. This will obtain a cluster with motif conductance of $O(k \phi)$ as shown in section~\ref{sec:motif_conductance_analysis}.


\subsection{HG-CRD Toy Example}

\begin{fullwidthfigure}
\includegraphics[width=\linewidth]{figures//crd_example.eps}
\caption{Explanation of hypergraph CRD (HG-CRD) steps on a toy example when we start the diffusion process from node $0$ and where each hyperedge (triangle in this case) has a maximum capacity of two. Note that red nodes are nodes with excess of flow, while black nodes are nodes with no excess. At the end, HG-CRD was able to highlight the correct cluster containing nodes 0, 1, 2 and 3.}
\label{fig:crd_toy_example}
\end{fullwidthfigure}

In this section, we will describe the hypergraph CRD dynamics on a toy example. Figure~\ref{fig:crd_toy_example} shows the motif-based degree and the flow for each node of the graph at each iteration. We will start the process from the seed node $0$ and let us choose the triangle as the motif we would like to consider in our clustering process. Additionally, we will fix each hyperedge maximum capacity $C$ to be two. At iteration $0$, node $0$ will increase its level by one in order to be able to push flow, then it will pick hyperedges $\{0,1,3\}$, $\{0,1,2\}$ and $\{0,2,3\}$ and push one unit of flow to each one of them. After that at iteration $1$, each node will double its flow value. In this iteration, only node $0$ has excess of flow and therefore it will again pick hyperedge $\{0,1,3\}$, $\{0,1,2\}$ and $\{0,2,3\}$ and push one unit of flow to each one of them. Similarly at iteration 2, each node will double its flow value. In this iteration, nodes $0, 1, 2$ and $3$ have excess of flow and therefore node $1$ will send two units of flow to hyperedge $\{1,4,6\}$ and will not be able to send more flow as the hyperedge has reached its maximum capacity (Recall that we have fixed the maximum capacity of each hyperedge to be two). In the rest of the iteration, node $0, 1, 2$ and $3$ will exchange the flow between them until their levels reach the maximum level $h$ and this will terminate the iteration. Finally, we have four nodes with excess and the detected cluster $A$ will be $0$, $1$, $2$ and $3$ as these nodes have $\vm_M \geq \vd_M$. In case of original CRD, the returned cluster $A$ will be nodes $0$, $1$, $2$, $3$ and $7$, as some flow will leak to node $7$.



\subsection{Motivating Example} \label{sec:motivation_example_localized}


One of the key advantages of CRD and our HG-CRD generalization is that they can provably explore a vastly smaller region of the graph than random walk or spectral methods. (Even those based on the approximate PageRank.) Here, figure~\ref{fig:motivation_example_leakage} shows a generalized graph of the graph provided in the original CRD paper \citep{wang2017capacity}, where we are interested in clustering this graph based on the triangle motif. In this graph, there are $p$ paths, each having $l$ triangles and each path is connected at the end to the vertex $u$ with a triangle. In higher order spectral clustering techniques, the process will require $\Omega(k^2l^2)$ steps to spread enough mass to cluster $B$. During these steps, the probability to visit node $v$ is $\Omega(k l/p)$. If $l = \Omega(p)$, then the random walk will escape from $B$. However, let us consider the worst case in HG-CRD where we start from $u$. In this case, $1/p$ of the flow will leak from $u$ to $v$ in each iteration. As HG-CRD process doubles the flow of the nodes in each iteration, it only needs $\text{log } l$ iterations to spread enough flow to cluster $B$ and therefore the flow leaking to $\bar{B}$ will be $(\text{log } l)/p$ of the total flow in the graph. This means HG-CRD will stay more localized in cluster $B$ and will leak flow to $\bar{B}$ much less than higher order spectral clustering techniques by a factor of $\Omega(\frac{p}{\text{log } l})$. HG-CRD is also able to detect the cluster in fewer number of iterations than higher order spectral clustering.


\begin{marginfigure}[-5\baselineskip]
\centering
\includegraphics[width=\linewidth]{figures//crd_motivation_example.eps}
\caption{Generalized example to show a comparison between hypergraph CRD (HG-CRD) and higher order spectral clustering. Starting the diffusion process from node $u$, HG-CRD will stay more localized in cluster $B$ and will leak flow to $\bar{B}$ much less than higher order spectral clustering techniques by a factor of $\Omega(\frac{p}{\text{log } l})$.}
\label{fig:motivation_example_leakage}
\end{marginfigure}


\subsection{HG-CRD Analysis} \label{sec:motif_conductance_analysis}
The analysis of CRD proceeds in a target recovery fashion. Suppose there exists a set $B$ with motif conductance $\phi$ and that is well-connected internally in a manner we will make precise shortly. This notion of internal connectivity is discussed at length in~\cite{wang2017capacity} and \cite{zhu2013local}. Suffice it to say, the internal connectivity constraints that are likely to be true for much of the social and information networks studied, whereas these internal connectivity constraints are not likely to be true for planar or grid-like data.  We show that HG-CRD, when seeded inside $B$ with appropriate parameters, will identify a set closely related to $B$ (in terms of precision and recall) with conductance at most $O(k \phi)$ where $k$ is the largest size of a hyperedge. Our theory heavily leverages the results from~\cite{wang2017capacity}. We restate theorems here for completeness and provide all the adjusted details of the proofs in the supplementary material. However, these should be understood as mild generalizations of the results -- hence, the statement of the theorems is extremely similar to~\cite{wang2017capacity}. Note that there are some issues with directly applying the proof techniques. For instance, some of the case analysis requires new details to handle scenarios that only arise with hyperedges. These scenarios are discussed in~\ref{hg-crd--theory-diff}.

\begin{theorem}[Generalization of \citet{wang2017capacity}, Theorem 1] \label{theorem:Theorem1_generalized}

Given G, $\vm_M$, $\phi \in (0, 1]$ such that: $\ve^T \vm_M \leq \text{volM}(G)$ and $\vm_M(v) \leq 2 \vd_M(v)$ $\text{ } \forall v \in V$ at the start, HG-CRD inner terminates with one of the following:
\begin{compactitem}
    \item \textbf{Case 1:} HG-CRD-inner finishes with $\vm_M(v) \leq  \vd_M(v) \text{ } \forall v \in V$,
    \item \textbf{Case 2:} There are nodes with excess and we can find cut A of motif-based conductance of O$(k \phi)$. Moreover, $2 \vd_M(v) \geq \vm_M(v)\geq \vd_M(v) \text{ } \forall v \in A \text{ and } \vm_M(v) \leq \vd_M(v) \text{ } \forall v \in \bar{A}$.
\end{compactitem}
\end{theorem}

Let us assume that there exists a good cluster $B$ that we are trying to recover. The goodness of cluster B will be captured by the following two assumptions, which are a generalized version of the two assumptions mentioned in CRD analysis:

\begin{assumption}
[Generalization of \citet{wang2017capacity}, Assumption 1]
\begin{align*}
\sigma_1 = \phi^{(s)}_M(B)/((k-1) \phi_M(B)) \geq \Omega(1),
\end{align*}
where $\phi^{(s)}_M(B)$ is the set motif conductance, which is defined as the minimum motif conductance of any set in the induced subgraph on $B$. This means that any subset in $B$ has worse motif conductance than the set $B$ by a gap of $k-1$, which makes $B$ a good cluster.
\end{assumption}

\begin{assumption}
[Generalization of \citet{wang2017capacity}, Assumption 2]

$\exists \text{  }\sigma_2 \geq \Omega(1) \text{, such that any } T \subset B \text{ having } \text{ volM} (T) \leq \text{volM} (B)/2 \text{, satisfies: }$
\begin{align*}
|M(T, B \setminus T)|/(|M(T, \bar{B})| \text{ log volM} (B) / \phi^{(S)}_M(B)) \geq \sigma_2,
\end{align*}
where $|M(A, B)|$ is the number of hyperedges with at least one endpoint in $A$ and at least another endpoint in $B$. This assumption states that any subset $T$ in $B$ is more connected via hyperedges to nodes in $B$ than nodes in $\bar{B}$ by a factor of $\sigma_2 \text{ log volM}(B)/\phi^{(S)}_M(B)$.
\end{assumption}

HG-CRD will work as follows, similar to CRD process, we will assume good cluster $B$ that satisfies assumption 1 and 2, and has the following properties: $\text{vol}_M (B) \leq \text{vol}_M(G)/2$, the diffusion will start from $v_s \in B$ and we know estimates of $\phi^{(S)}_M (B)$ and $\text{vol}_M (B)$ and we will set $\phi = \theta(\phi^{(S)}_M (B)/k)$.

\begin{theorem} [Generalization of \citet{wang2017capacity}, Theorem 3] \label{theorem:Theorem3_generalized}

If we run HG-CRD with $\phi \geq \Omega(\phi_M(B))/k$, then:
\begin{compactitem}
    \item  $\text{vol}_M (A \setminus B) \leq O(k/\sigma) . \text{vol}_M(B)$ ,
    \item  $\text{vol}_M (B \setminus A) . \leq O(k/\sigma) \text{vol}_M(B)$,
    \item $\phi_M(A) \leq O(k \phi)$,
\end{compactitem}
 where $A = \{v \in V| d_M(v) \leq m_M(v) \}$ and $\sigma = min(\sigma_1, \sigma_2)$.
\end{theorem}

\subsection{Theoretical Challenges} \label{hg-crd--theory-diff}
Proving the previous theorems for HG-CRD is non-trivial since several cases arises in hyperedges that do not exist in the original CRD. In this subsection, we discuss some of these non-trivial cases (The complete proofs of the theorems are provided in the supplementary material), such as:
\begin{compactitem}
    \item Theorem~\ref{theorem:Theorem1_generalized}: To prove this theorem, CRD~\citep{wang2017capacity} groups nodes based on their level value (nodes in level $i$ will be in group $B_i$) and then consider nodes with level at least $i$ to be in one cluster ($S_i$). After that, they categorize edges between cluster $S_i$ and $\bar{S}_i$ into two groups based on the level values of their endpoints. Since hyperedges do not have two endpoints, we needed to extend this categorization and proved similar properties for the extension. Because of this extension, we got a gap of $k$ between the motif conductance and $\phi$ as we proved that the motif conductance is $O(k \phi)$ instead of the original proof where the conductance is $O(\phi)$.
    \item Theorem~\ref{theorem:Theorem3_generalized}: The proof of CRD~\citep{wang2017capacity} relies on the following equation: 
    \begin{align*}
        \sum_{i=1}^h |E(B_i, \bar{B})| \min(i, 1/\phi)=   \sum_{i=1}^{1/\phi} |E(S_i, \bar{B})| ,
    \end{align*}
 where $E(A, B)$ is the set of edges from cluster $A$ to cluster $B$. This equation only holds for edges and not true for hyperedges of $k > 2$. Therefore, we provide a totally different proof that works for hyperedges of any sizes.
\end{compactitem}

\subsection{Running Time and Space Discussion.}
The running time of local algorithms are usually stated in terms of the output.
Recall that CRD running time is $O((\text{vol}(A) \text{ log vol} (A))/\phi)$. As hypergraph CRD replaces the degree of vertices by the motif-based degree and the flow in each iteration depends on the motif-based degree, therefore the running time will depend on $\text{volM}(A)$ instead of $\text{vol}(A)$ and it will be $O((\text{volM}(A) \text{ log volM} (A)) /\phi)$. For space complexity, it is $O(\text{volM}(A))$, as each node $v$ we explore in our local clustering will store hyperedges containing it. 

==> sources/cut-text.tex <==



\textbf{Old text, can take bits as appropriate...}


Diffusion methods have been widely applied to a large variety of graph mining tasks~\cite{pan2004-cross-modal-discovery,Gleich-2015-prbeyond,Gleich-2016-mining,chung2007heat,Li-2015-lemon,Joachims-2003-transductive}. The basic intuition behind these methods is to start from seed nodes and then spread the mass from the nodes to their neighbors according to some rules described by the diffusion process. For example, heat diffusion \cite{chung2007heat} spread the mass based on a differential equation, max-flow quotient-cut improvement (MQI) \cite{lang2004flow}, Flow-Improve \cite{andersen2008algorithm} and Local Flow-Improve \cite{orecchia2014flow} spread the mass using flow-based techniques, personalized PageRank \cite{andersen2006local} spread the mass according to an iterative equation. These traditional diffusion methods are subject to the quadratic Cheeger inequality, which states that the conductance of the detected cluster is within a quadratic factor of the optimal conductance. Recently, a new method called capacity releasing diffusion (CRD) process was proposed. This diffusion method was shown to be faster and stays more locally than the traditional spectral diffusions. Moreover, CRD is the first local graph clustering technique that is not subject to the quadratic Cheeger inequality by assuming the existence of a good cluster near the seed nodes.

Furthermore, higher order patterns are important components in understanding complex networks. They appear in many applications, for example as shown by  Benson et al.~\cite{benson2016higher}, social networks are rich of triangular patterns, airline traffic behaviour are better analyzed using two-hop paths and feed forward loops are important blocks in understanding regulation networks. Recent techniques are proposed to extend traditional clustering techniques \cite{benson2016higher, tsourakakis2017scalable, li2017inhomogeneous} to account for higher order patterns like motifs (small sub graphs). These techniques aim to cluster the whole graph based on motifs instead of edges. Additionally, Yin et al. \cite{yin2017local} explored the usage of higher order patterns in performing local graph clustering, by extending the approximate personalized PageRank (APPR) to cluster based on motifs. Motif-based approximate personalized PageRank (MAPPR) was shown experimentally to enhance the quality of the returned communities in the community detection task.

